Explore User Neighborhood for Real-time E-commerce Recommendation

Recommender systems play a vital role in modern online services, such as Amazon and Taobao. Traditional personalized methods, which focus on user-item (UI) relations, have been widely applied in industrial settings, owing to their efficiency and effectiveness. Despite their success, we argue that these approaches ignore local information hidden in similar users. To tackle this problem, user-based methods exploit similar user relations to make recommendations in a local perspective. Nevertheless, traditional user-based methods, like userKNN and matrix factorization, are intractable to be deployed in the real-time applications since such transductive models have to be recomputed or retrained with any new interaction. To overcome this challenge, we propose a framework called self-complementary collaborative filtering~(SCCF) which can make recommendations with both global and local information in real time. On the one hand, it utilizes UI relations and user neighborhood to capture both global and local information. On the other hand, it can identify similar users for each user in real time by inferring user representations on the fly with an inductive model. The proposed framework can be seamlessly incorporated into existing inductive UI approach and benefit from user neighborhood with little additional computation. It is also the first attempt to apply user-based methods in real-time settings. The effectiveness and efficiency of SCCF are demonstrated through extensive offline experiments on four public datasets, as well as a large scale online A/B test in Taobao.

==> input_embedding.tex <==
\subsubsection{Input Layer}
For non-sequential models, given the ID feature of item set $\mathcal{R}_u^+$, one-hot encoding is applied to represent this sort of input. 
Since the information delivered by the sparse one-hot vector is limited, we adopt an embedding mechanism to map the vector to an informative and lower-dimensional vector representation. 
In this way, for each historical item $i \in \mathcal{R}_u^+ $, we project it to an embedding vector $\bm{p}_i \in \mathbb{R}^k$. 
Therefore, the output of the input layer is a set of vectors $\mathcal{P}_u = \{\bm{p}_i|i\in\mathcal{R}_u^+\}$. And the input embedding matrix $\bm{P} \in \mathbb{R}^{k \times m}$ is the total embedding of all items in $\mathcal{I}$. 

When it comes to sequential models, we need to take the position information into account together with the ID feature of items. Here, we inject a position embedding $\bm{E} \in \mathbb{R}^{k \times m}$ into the input embedding vectors. Thus, the output of the input layer is a sequence of embedding: 

\begin{equation}
\hat{\bm{S}}_u = 
\begin{bmatrix}
    (\bm{p}_{i_1^{(u)}}+\bm{e}_1)^T \\
    (\bm{p}_{i_2^{(u)}}+\bm{e}_2)^T \\
    \dots \\
    (\bm{p}_{i^{(u)}_{|\mathcal{S}^u|}} + \bm{e}_{|\mathcal{S}^u|})^T.
\end{bmatrix}
\end{equation}
Here, instead of fixed embedding, we adopt the learnable position embedding for better performance since it allows our model to identify which portion of the input it handles~\cite{vaswani2017attention}. 
However, it also induces a restriction on the maximum sequence length $N$ that sequential models can cope with. 
To alleviate the problem, if $|\mathcal{S}^u| > N$, we truncate the input sequence $\mathcal{S}_u$ to the last $N$ items:
\begin{equation}
    \mathcal{S}_u=[i_{|\mathcal{S}^u|-N + 1}^{(u)},i_{|\mathcal{S}^u|-N+2}^{(u)},\dots,i^{(u)}_{|\mathcal{S}^u|}].
\end{equation}

Besides ID features and position information, the input layer can be easily extended to incorporate side information, such as item attributes. 
However, since this work focuses on the collaborative filtering setting, here we do not consider the incorporation of side information.

==> table_no_use.tex <==
\begin{table}
\setlength{\tabcolsep}{0.7em}
    \centering
    \caption{Performance comparison of different embedding sizes on top-$N$ recommendation. Bold scores are the best in method group. Improvements are calculated over U2I methods.} %
        \begin{tabular}{ ll c c c c}
        \toprule
        Size & Datasets & U2I & U2U & SCCF & Improv. \\
        \midrule
        \multirow{3}{*}{size=8} 
        & ML-1M & 0.2953 & 0.3311 & 0.3460 & 17.17\% \\
        
         & Games & 0.1490 & 0.1258 & 0.1856 & 24.56\%\\
         
         & Beauty & 0.0496 & 0.0431 & 0.0660 & 33.06\%\\
         
         \midrule
        \multirow{3}{*}{size=16} & 
        ML-1M & 0.3955 & 0.3880 & 0.4223 & 6.77\%\\
         
         & Games & 0.1984 & 0.1577 & 0.2212 & 11.49\% \\
         
         & Beauty & 0.0519 & 0.0549 & 0.0733 & 41.23\%\\
         
         \midrule
        \multirow{3}{*}{size=64} 
        & ML-1M & 0.5200 & 0.4301 & 0.4834 & ~~-7.57\% \\
         
         & Games & 0.2230 & 0.2035 & 0.2335 & ~~4.71\% \\
         
         & Beauty & 0.0902 & 0.0857 & 0.0936 & 3.77\%\\
        \bottomrule
        \end{tabular}
    \label{tab:hyper}
\end{table}
